Low-Complexity Switch Scheduling Algorithms: Delay Optimality in Heavy Traffic

Motivated by applications in data center networks, in this paper, we study the problem of scheduling in an input queued switch. While throughput maximizing algorithms in a switch are well-understood, delay analysis was developed only recently. It was recently shown that the well-known MaxWeight algorithm achieves optimal scaling of mean queue lengths in steady state in the heavy-traffic regime, and is within a factor less than $2$ of a universal lower bound. However, MaxWeight is not used in practice because of its high time complexity. In this paper, we study several low complexity algorithms and show that their heavy-traffic performance is identical to that of MaxWeight. We first present a negative result that picking a random schedule does not have optimal heavy-traffic scaling of queue lengths even under uniform traffic. We then show that if one picks the best among two matchings or modifies a random matching even a little, using the so-called flip operation, it leads to MaxWeight like heavy-traffic performance under uniform traffic. We then focus on the case of non-uniform traffic and show that a large class of low time complexity algorithms have the same heavy-traffic performance as MaxWeight, as long as it is ensured that a MaxWeight matching is picked often enough. We also briefly discuss the performance of these algorithms in the large scale heavy-traffic regime when the size of the switch increases simultaneously with the load. Finally, we perform empirical study on a new algorithm to compare its performance with some existing algorithms.

==> Class_discussion.tex <==
%!TEX root = main.tex

\color{blue}
\section{Discussion on Classes}

So far, we studied the performance of three classes of algorithms. In this section, we present a short discussion about them. The three classes are clearly not disjoint. For instance, as mentioned before, MaxWeight lies in all three classes. It is not hard to construct other algorithms that lie in all three classes. one can combine multiple scheduling algorithms to generate a new algorithm. 
%Note that for switch system, one can combine multiple scheduling algorithms to generate a new algorithm. 
For example, one can create a scheduling algorithm that generate two schedules, one by bursty MaxWeight and other by power-of-$d$ and then chooses the one with higher weight. Such an algorithm will lie in both class $\Pi_1(\frac{1}{n} \mathbf{1})$ and $\Pi_2$. Another example is PC-$d$ (Section \ref{sec: randomly_delayed_maxweight}), which was created by implementing an extra comparison step after doing power-of-$d$. So PC-$d$ lie in both $\Pi_{1}(\frac{1}{n} \mathbf{1})$ and $\Pi_3$. A similar modification  can be done with random $d$-flip without changing the complexity of the algorithm. 

While we proved that they all have MaxWeight-like heavy-traffic mean delay performance, their performance under other metrics can be different. 
%We looked at three classes of algorithm and proved that their \htlike. Although this does not imply that their performance is similar moderate traffic. As mentioned before, 
First consider throughput optimality. As mentioned before, while 
the algorithms in class $\Pi_2$ and class $\Pi_3$ are throughput optimal, %(i.e., the switch system is stable under any arrival rate matrix in the capacity region $\mathcal{C}$), 
the algorithms in $\Pi_1(\nu)$ are not. 
%. Same cannot be said for algorithms in class $\Pi_1(\nu)$. 
Power-of-$d$ and random $d$-flip are known to be stable only in a subset of the capacity region $\mathcal{C}^*$. 
In particular, they support maximum possible load only when the traffic is uniform. There are known examples \siva{\cite{}} showing how they are unstable under non-uniform load for certain arrival rate vectors within the capacity region. 
%ey are maximally stable only under uniform traffic. So in terms of throughput, algorithms in class $\Pi_2$ and class $\Pi_3$ are better than algorithms in class $\Pi_1(\nu)$. 

% Large scale heavy-traffic regimes provide other performance metrics to distinguish between various classes. While \siva{Theorem ??} clearly shows the difference in performance of algorithms in various classes, we point out that we do not know a  
% As stated in \siva{Theorem ??}, 
% In large scale heavy traffic regime also, for the examples considered in this paper, the algorithms in class $\Pi_2$ perform better than the algorithms considered in class $\Pi_1(\nu)$. As mentioned before, the time complexities of  power-of-$d$ and random $d$-flip are linear in $n$. And for them, we need $\beta >6$ (Given in Sec. \ref{sec: large_scale_po2}). For bursty MaxWeight, time complexity is $O(n^3/m)$. So, if we choose $m=n^2$,  the time complexity is linear in $n$ and then $\gamma = 2$ and so  we need $\beta>5$ (Given in Sec. \ref{sec: large_scale_bursty}). This gives the idea that  bursty MaxWeight is better than power-of-$d$ and random-$d$-flip in large scale heavy traffic regime.



